Pixels to Plans: Learning Non-Prehensile Manipulation by Imitating a Planner

We present a novel method enabling robots to quickly learn to manipulate objects by leveraging a motion planner to generate "expert" training trajectories from a small amount of human-labeled data. In contrast to the traditional sense-plan-act cycle, we propose a deep learning architecture and training regimen called PtPNet that can estimate effective end-effector trajectories for manipulation directly from a single RGB-D image of an object. Additionally, we present a data collection and augmentation pipeline that enables the automatic generation of large numbers (millions) of training image and trajectory examples with almost no human labeling effort. We demonstrate our approach in a non-prehensile tool-based manipulation task, specifically picking up shoes with a hook. In hardware experiments, PtPNet generates motion plans (open-loop trajectories) that reliably (89% success over 189 trials) pick up four very different shoes from a range of positions and orientations, and reliably picks up a shoe it has never seen before. Compared with a traditional sense-plan-act paradigm, our system has the advantages of operating on sparse information (single RGB-D frame), producing high-quality trajectories much faster than the "expert" planner (300ms versus several seconds), and generalizing effectively to previously unseen shoes.

==> discussion.tex <==
%auto-ignore
The results of our experiments suggest that semi-supervised imitation learning using a kinematic motion planner as a supervision signal is a relatively robust, data-efficient method for single-view estimation of end-effector trajectories for the examined manipulation task, using only 34 human-generated annotations. Further, we posit that the method should generalize to other manipulation tasks in which collision avoidance is important but only partial state observations are available.

% Compared to \SGNet, these RRT trajectories use a high quality 3D model of the shoe. Although sampling-based planning can find a feasible solution very fast in a complicated environment, it has a weakness that it requires very accurate environment model for collision check. However, in real application, it is impossible to construct the accurate model for collision check from real time sensor information. Therefore, we train \SGNet with these RRT trajectories with high-quality model for \SGNet to generate trajectories without the full high-quality model information. In addition, since \SGNet can generate the trajectory very fast compared to sampling-based planning without full information, it is very valuable advantage. 

%In the time of system implementation, we were able to observe three main factors that cause a performance degradation, deformation of the shoe shape, misalignment of camera and robot coordinate frame, and noisy segmentation. During the experiments, the most failure cases were caused by collisions between the hook and the surrounding structure of the shoe entrance.
However, the learned system has several clearly defined, repeatable failure modes. For example, we observed that system performance was sensitive to the quality of the segmentation: poor shoe segmentation results often lead the system to failure. There are two primary avenues to addressing this issue, including a) increasing the robustness of \SGNet to bad segmentations and/or b) eliminate the need for masking. Significant progress could be made on both fronts through data augmentation, replacing the backgrounds with random scenes and distractors for robustness. However, the use of segmentations are useful to our system in that they serve as a convenient attention mechanism, allowing the network to estimate trajectories for scenes containing multiple objects of interest by selectively masking them. Further, as demonstrated in Section~\ref{sec:generalization-across-roll}, the network has only a limited ability to generalize to unseen shoe poses. This is largely due to the range of camera positions used during data collection and could be mitigated by acquiring more complete coverage of the hemisphere of possible camera positions during data collection. In general, when the system fails, it fails because the end-effector collides with the outside of the shoe.

%Our results suggest several possible paths for future work. A more comprehensive test containing broader manipulation tasks and classes of objects would help better demonstrate the generality of our method. In addition, more experimentation is needed to determine an effective trade-off between neural network architecture size and computational demands; for true real-time trajectory estimation, a more compact architecture backbone is needed. 

%A possible issue with our method is the use of a sampling-based planner for generating ground truth. If two similar input pairs to the network have similar and non-convex solution spaces, the stochasticity in the ground truth produced by a sampling-based planner might produce undesirable behavior when coupled with the minimization of an L1 or L2 penalty in the network's loss function. For example, the task of picking up a flip-flip sandal with two straps has a non-convex solution in the sense that selecting either loop for hooking will be successful, but the `average' of these two might collide with the strap separating them. To address this shortcoming, we might use a variational method as in as in \cite{journals/corr/HoE16} to estimate the parameters of the data-generating distribution itself, making the probability of selecting an incorrect `average' solution relatively small.

==> old-intro.tex <==
%auto-ignore
% This is a very learning-oriented introduction to our work; adding something more robotics/tool-oriented might be helpful

%% Here is the robotics guy's take on it
Despite many advances in robotic manipulation in industrial settings, manipulating general objects in unstructured environment is still challenging.
Recent deep learning approaches have proven well-suited to address related challenges (e.g. background and light variation) in computer vision tasks such as object detection and recognition.  Even though these advances directly improve the ``sense" component of the classical sense-plan-act cycle of manipulation, the requirement to hard code explicit representations between these components adversely affects the robustness of approaches which keep them separate.





%Real-world robotics tasks have proven well-suited for evaluating the limits of modern deep learning methods in terms of data efficiency, computational requirements, and generalization ability. 
In the context of manipulation, recent `pixels-to-actions' methods have shown some promise in estimating effective actions in the form of joint angles or torques directly from raw sensor data, without any explicit intermediate state \cite{DBLP:journals/corr/LevineFDA15} \cite{DBLP:journals/corr/LevinePKQ16}. These methods are very flexible and can run in real-time settings. However, current pixels-to-actions techniques have limitations: they often suffer from both high sample complexity and brittleness in the presence of deviations from the learning environment, which are particularly significant in the context of robotics. In contrast, the traditional `sense-plan-act' solution to a manipulation task might perform some state estimation from the geometry and/or visual features or the object of interest (potentially with a convolutional neural network) and then execute an action plan from a motion planner. This approach to the problem is data efficient and generalizes very well but demands high-fidelity state information, the computational demands of which might make these strategies impractical for truly real-time systems. 

This work proposes a hybrid approach to manipulation tasks that combines the \textbf{robustness} and \textbf{data efficiency} of traditional motion planners when provided with high fidelity state information and the \textbf{flexibility} and \textbf{speed} of neural networks when provided with raw sensor data. More concretely, we present a system for robustly picking up shoes with a hooking tool.

We demonstrate this approach in the context of a tool-based manipulation task, specifically picking up shoes with a hook tool.  Using a passive (unactuated) tool end-effector in place of traditional actuated grippers provides benefits in terms of robustness to damage, low cost, and simplicity.  
Compared to traditional actuated grippers, passive (unactuated) tools are simple, robust to damage, and low-cost.  Humans demonstrate remarkable dexterity in manipulating objects with tools, and frequently opt to use tools preferentially over their hands for common manipulation tasks (e.g. eating).   

This system includes an automated data collection and ground truth generation pipeline that requires very little human intervention, making datasets with hundreds of thousands of samples practical to produce. Using this pipeline, our system trains a neural network to produce end-effector trajectories (in the frame of the camera) from raw RGBD data that imitate the output of an RRT motion planner. Leveraging the relatively slow but precise motion planner at train time, we show that we can learn to reliably hook even previously unseen shoes without access to a 3D model or motion planner at test time.

% To assess our method, we present two systems for manipulating shoes with a hooking tool. One system, which we propose as a Tools are useful for manipulating objects robustly and cheaply. Many animals make use of tools to augment their naturally-endowed physical capabilities, from crows to primates \cite{Hunt1996} \cite{Mulcahy2006}. We claim that endowing robots with a similar ability to understand object affordances with respect to available tools is a critical step in making them practical for everyday manipulation-heavy tasks. In this work, we propose a general framework for learning this ability for a significant subset of such manipulation tasks, specifically, those tasks that can be solved with a kinematic motion planner given enough time, information, and compute resources. More concretely, we present a system that implements this learning and manipulation framework for the task of picking up a diverse set of shoes with a hook.  Using this collection framework, we train a neural network to infer an effective trajectory for picking up a shoe with a hook from a single viewpoint.

% \begin{itemize}
% \item Semi-supervised learning to go from pixels to a shoe-hooking actions
% \item Tool based manipulation - A low-cost, interesting/underexplored strategy for picking up objects. \ttxt{TODO: Tarik needs to add a motivation paragraph for tool-based manipulation}
% \item Picking up a shoe with a hook is basically a \textbf{kinematic planning} task: the hard part is figuring out how to get the hook into the shoe without colliding with the shoe
% \item Given perfect knowledge of the shoe's \textbf{geometry} and \textbf{pose} relative the robot, a hooking trajectory can be generated using a black box motion planner
% \item However, if all we have is a \textbf{single rgbd view} of the shoe, it is not possible to infer the whole geometry directly.
% \item We are training a network to infer the \textbf{correct hooking trajectory} (generated by a planner with high-quality geometric data) from a \textbf{single rgbd image}
%\vtxt{here scale will be an issue. We need to articulate the assumption we make about it. I can think of i) the shoes are more or less the same size and the network is robust enough for variantions of size. ii) it learns actions specific to some subset of shoes -- e.g. if we had the same shoe size 6 and size 13, it won't work}.
% \end{itemize}


% \emph{Our contributions can be summarized as follows.}

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/hook.jpg}
    \caption{Hook tool used by the robot to manipulate shoes}
    \label{fig:hook}
\end{figure}


traditional: sense-plan-act
ours: computatio
al efficiency, better generalizatinno
ours: sense-plan

end-to-end: a lot of examples and good model of the tool; good dynamic model fro
 many examples; not clear how it generalizes e.g. in the arm farm pa
er

too tight coupling
p
m
